Pervasive Cloud Controller for Geotemporal Inputs

The rapid cloud computing growth has turned data center energy consumption into a global problem. At the same time, modern cloud providers operate multiple geographically-distributed data centers. Distributed data center infrastructure changes the rules of cloud control, as energy costs depend on current regional electricity prices and temperatures. Furthermore, to account for emerging technologies surrounding the cloud ecosystem, a maintainable control solution needs to be forward-compatible. Existing cloud controllers are focused on VM consolidation methods suitable only for a single data center or consider migration just in case of workload peaks, not accounting for all the aspects of geographically distributed data centers. In this paper, we propose a pervasive cloud controller for dynamic resource reallocation adapting to volatile time- and location-dependent factors, while considering the QoS impact of too frequent migrations and the data quality limits of time series forecasting methods. The controller is designed with extensible decision support components. We evaluate it in a simulation using historical traces of electricity prices and temperatures. By optimising for these additional factors, we estimate 28.6% energy cost savings compared to baseline dynamic VM consolidation. We provide a range of guidelines for cloud providers, showing the environment conditions necessary to achieve significant cost savings and we validate the controller's extensibility.

==> dodatno/abbrev.tex <==
% special expressions:
\newcommand{\coe}{$CO_{2}e$}

%constants
\newcommand{\numdays}{120}
\newcommand{\pricefluct}{0.1}
%\newcommand{\eqtopmargin}{-0.5cm}
\newcommand{\eqtopmargin}{-0.1cm}
%\newcommand{\eqbottommargin}{-0.5cm}
\newcommand{\eqbottommargin}{-0.3cm}
\newcommand{\eqtopmarginbig}{-0.4cm}
\newcommand{\eqbottommarginbig}{-0.4cm}
\newcommand{\tabletopmargin}{-0.3cm}
\newcommand{\tablecaptionmargin}{-0.2cm}
\newcommand{\tablebottommargin}{-0.1cm}
\newcommand{\figtopmargin}{-0.2cm}
\newcommand{\figbottommargin}{-0.5cm}
\newcommand{\figcaptionmargin}{-0.7cm}


\newacronym{coe}{\coe}{$CO_{2}$ equivalent}
\newacronym{ewma}{EWMA}{exponentially weighted moving average}
\newacronym{dvfs}{DVFS}{dynamic voltage \& frequency scaling}
\newacronym{vm}{VM}{virtual machine}
\newacronym{era}{ERA}{energy reduction assets}
\newacronym{api}{API}{application programming interface}
\newacronym{os}{OS}{operating system}
\newacronym{rtp}{RTP}{real-time pricing}
\newacronym{qos}{QoS}{quality of service}
\newacronym{sla}{SLA}{service level agreement}
\newacronym{rtep}{RTEP}{real-time electricity pricing}
\newacronym{iaas}{IaaS}{infrastructure as a service}
\newacronym{pm}{PM}{physical machine}
\newacronym{pue}{PUE}{power usage efficiency}
\newacronym{cue}{CUE}{carbon usage effectiveness}
\newacronym{cef}{CEF}{carbon emission factor}
\newacronym{hpc}{HPC}{high-performance computing}
\newacronym{db}{DB}{database}
\newacronym{dc}{DC}{data center}
\newacronym{oltp}{OLTP}{online transaction processing}
\newacronym{mse}{MSE}{mean squared error}
\newacronym{ga}{GA}{genetic algorithm}
\newacronym{arima}{ARIMA}{autoregressive integrated moving average}
\newacronym{ses}{SES}{simple exponential smoothing}
\newacronym{bcf}{BCF}{best cost fit}
\newacronym{bfd}{BFD}{best fit decreasing}
\newacronym{iot}{IoT}{Internet of Things}

==> dodatno/reviews1/review_response/abbrev.tex <==
% special expressions:
\newcommand{\coe}{$CO_{2}e$}

%constants
\newcommand{\numdays}{120}
\newcommand{\pricefluct}{0.1}
%\newcommand{\eqtopmargin}{-0.5cm}
\newcommand{\eqtopmargin}{-0.1cm}
%\newcommand{\eqbottommargin}{-0.5cm}
\newcommand{\eqbottommargin}{-0.3cm}
\newcommand{\eqtopmarginbig}{-0.4cm}
\newcommand{\eqbottommarginbig}{-0.4cm}
\newcommand{\tabletopmargin}{-0.3cm}
\newcommand{\tablecaptionmargin}{-0.2cm}
\newcommand{\tablebottommargin}{-0.1cm}
\newcommand{\figtopmargin}{-0.2cm}
\newcommand{\figbottommargin}{-0.5cm}
\newcommand{\figcaptionmargin}{-0.7cm}


\newacronym{coe}{\coe}{$CO_{2}$ equivalent}
\newacronym{ewma}{EWMA}{exponentially weighted moving average}
\newacronym{dvfs}{DVFS}{dynamic voltage \& frequency scaling}
\newacronym{vm}{VM}{virtual machine}
\newacronym{era}{ERA}{energy reduction assets}
\newacronym{api}{API}{application programming interface}
\newacronym{os}{OS}{operating system}
\newacronym{rtp}{RTP}{real-time pricing}
\newacronym{qos}{QoS}{quality of service}
\newacronym{sla}{SLA}{service level agreement}
\newacronym{rtep}{RTEP}{real-time electricity pricing}
\newacronym{iaas}{IaaS}{infrastructure as a service}
\newacronym{pm}{PM}{physical machine}
\newacronym{pue}{PUE}{power usage efficiency}
\newacronym{cue}{CUE}{carbon usage effectiveness}
\newacronym{cef}{CEF}{carbon emission factor}
\newacronym{hpc}{HPC}{high-performance computing}
\newacronym{db}{DB}{database}
\newacronym{dc}{DC}{data center}
\newacronym{oltp}{OLTP}{online transaction processing}
\newacronym{mse}{MSE}{mean squared error}
\newacronym{ga}{GA}{genetic algorithm}
\newacronym{arima}{ARIMA}{autoregressive integrated moving average}
\newacronym{ses}{SES}{simple exponential smoothing}
\newacronym{bcf}{BCF}{best cost fit}
\newacronym{bfd}{BFD}{best fit decreasing}
\newacronym{iot}{IoT}{Internet of Things}

==> dodatno/reviews1/review_response/response_macros.tex <==
\newcommand{\initresponses}{\newcounter{pointcounter}}

\newenvironment{reviewer}{\setcounter{pointcounter}{1}}{}

\newcommand{\point}[1]{\medskip \noindent
               \textsl{{\fontseries{b}\selectfont Q\thepointcounter}.
                 \stepcounter{pointcounter} #1}}
\newcommand{\reply}{\medskip \noindent \textbf{Answer}.\ }

